Modular Object-Oriented Games: A Task Framework for Reinforcement Learning, Psychology, and Neuroscience

In recent years, trends towards studying simulated games have gained momentum in the fields of artificial intelligence, cognitive science, psychology, and neuroscience. The intersections of these fields have also grown recently, as researchers increasing study such games using both artificial agents and human or animal subjects. However, implementing games can be a time-consuming endeavor and may require a researcher to grapple with complex codebases that are not easily customized. Furthermore, interdisciplinary researchers studying some combination of artificial intelligence, human psychology, and animal neurophysiology face additional challenges, because existing platforms are designed for only one of these domains. Here we introduce Modular Object-Oriented Games, a Python task framework that is lightweight, flexible, customizable, and designed for use by machine learning, psychology, and neurophysiology researchers.

==> macros.tex <==

%*********For this paper***********
\newcommand{\deriv}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand\cut[1]{}


\renewcommand{\L}{\mathcal{L}}
\newcommand{\enc}{\text{enc}}
\newcommand{\dec}{\text{dec}}
\newcommand{\utext}[2]{\underbrace{#1}_{\text{#2}}}

\newcommand{\betavae}{\ensuremath{\beta}-VAE\xspace}
\newcommand{\kldiv}{D_{KL}\divx}
\newcommand{\concept}[1]{\texttt{\{#1\}}}
\newcommand{\sym}[1]{\enquote{#1}}
\newcommand{\operator}[1]{\textsc{#1}}


\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}

%% densify spacing in bibliographies
\newcommand{\bibfix}{%    PUT \bibfix in file.bbl after first line
    \setlength{\parsep}{\parskip}%
    \setlength{\itemsep}{0cm}%
    \setlength{\topsep}{\parskip}%
    \setlength{\parskip}{0cm}%
    \setlength{\partopsep}{0cm}%
    \setlength{\listparindent}{\parindent}%
    \setlength{\labelwidth}{10pt}%
    \setlength{\labelsep}{0pt}%
    \setlength{\leftskip}{0pt}%
    \setlength{\leftmargin}{0pt}%
}

%Saving space: see
%   http://www-h.eng.cam.ac.uk/help/tpl/textprocessing/squeeze.html

%Page layout info:
%   http://amath.colorado.edu/documentation/LaTeX/reference/layout.html


% New column types for wrapped with alignments
\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}m{#1}}

\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}
\newenvironment{myproof}{{\bf Proof}}{}

\newcommand{\tm}{\tilde{m}}
\newcommand{\tv}{\tilde{v}}

\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\given}{\|}
\newcommand{\indep}[2]{{#1} \perp {#2}}
\newcommand{\condindep}[3]{{#1} \perp {#2} | {#3}}
\newcommand{\condindepG}[3]{{#1} \perp_G {#2} | {#3}}
\newcommand{\condindepP}[3]{{#1} \perp_p {#2} | {#3}}
\newcommand{\depend}[2]{{#1} \not \perp {#2}}
\newcommand{\conddepend}[3]{{#1} \not \perp {#2} | {#3}}

\newcommand{\trans}[1]{{#1}^{\mathtt{T}}}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\la}{\leftarrow}
\newcommand{\tr}{\mbox{tr}}

\newcommand{\dom}{\mbox{dom}}
\newcommand{\bel}{\mbox{bel}}
\newcommand{\dsep}{\mbox{dsep}}
\newcommand{\sep}{\mbox{sep}}
\newcommand{\entails}{\models}
\newcommand{\range}{\mbox{range}}
\newcommand{\myspan}{\mbox{span}}
\newcommand{\nullspace}{\mbox{nullspace}}
\newcommand{\adj}{\mbox{adj}}

\newcommand{\nbd}{\mbox{nbd}}
\newcommand{\nbr}{\mbox{nbr}}
\newcommand{\anc}{\mbox{anc}}
\newcommand{\desc}{\mbox{desc}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\nondesc}{\mbox{nondesc}}
\newcommand{\pa}{\pi}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\mb}{\mbox{mb}}
\newcommand{\connects}{\sim}


\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\NegBinom}{\mbox{NegBinom}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\cauchy}{\mbox{Cauchy}}
\newcommand{\DE}{\mbox{DE}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\calM}
\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\expon}{\mbox{Expon}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{{\cal N}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\IGauss}{\mbox{InvGauss}}
\newcommand{\IW}{\mbox{IW}}
\newcommand{\Laplace}{\mbox{Lap}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\GIG}{\mbox{NIG}}
\newcommand{\NIW}{\mbox{NIW}}
\newcommand{\GIW}{\mbox{NIW}}
\newcommand{\MVNIW}{\mbox{NIW}}
\newcommand{\NW}{\mbox{NWi}}
\newcommand{\MVNIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{{\cal T}}
\newcommand{\student}{{\cal T}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}
\newcommand{\unif}{\mbox{U}}
\newcommand{\etr}{\mbox{etr}}


\newcommand{\softmax}{\calS}
\newcommand{\soft}{\mbox{soft}}
\newcommand{\cond}{\mbox{cond}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{{\sc MATLAB}}
\newcommand{\NETLAB}{{\sc NETLAB}}
\newcommand{\MLABA}{\mbox{PMTK}}
\newcommand{\BLT}{\mbox{PMTK}}
\newcommand{\PMTK}{\mbox{PMTK}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\KLpq}[2]{\mathbb{KL}\left({#1}||{#2}\right)}
\newcommand{\KL}{\mbox{KL}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MIxy}[2]{\mathbb{I}\left({#1};{#2}\right)}
\newcommand{\MIxyz}[3]{\mathbb{I}\left({#1};{#2}|{#3}\right)}
\newcommand{\entropy}[1]{\mathbb{H}\left({#1}\right)}
\newcommand{\entropypq}[2]{\mathbb{H}\left({#1}, {#2}\right)}


\newcommand{\myvec}[1]{\boldsymbol{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\ind}[1]{\mathbb{I}(#1)}

\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}

\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vxi}{\myvecsym{\xi}}


\newcommand{\vmuY}{\vb}
\newcommand{\vmuMu}{\vmu_{x}}
\newcommand{\vmuMuGivenY}{\vmu_{x|y}}
\newcommand{\vSigmaMu}{\vSigma_{x}}
\newcommand{\vSigmaMuInv}{\vSigma_{x}^{-1}}
\newcommand{\vSigmaMuGivenY}{\vSigma_{x|y}}
\newcommand{\vSigmaMuGivenYinv}{\vSigma_{x|y}^{-1}}
\newcommand{\vSigmaY}{\vSigma_{y}}
\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

\newcommand{\muY}{\mu_{y}}
\newcommand{\muMu}{\mu_{\mu}}
\newcommand{\muMuGivenY}{\mu_{\mu|y}}
\newcommand{\SigmaMu}{\Sigma_{\mu}}
\newcommand{\SigmaMuInv}{\Sigma_{\mu}^{-1}}
\newcommand{\SigmaMuGivenY}{\Sigma_{\mu|y}}
\newcommand{\SigmaMuGivenYinv}{\Sigma_{\mu|y}^{-1}}
\newcommand{\SigmaY}{\Sigma_{y}}
\newcommand{\SigmaYinv}{\Sigma_{y}^{-1}}

\newcommand{\hatf}{\hat{f}}
\newcommand{\haty}{\hat{y}}
\newcommand{\const}{\mbox{const}}
\newcommand{\sigmoid}{\mbox{sigm}}

\newcommand{\one}{(1)}
\newcommand{\two}{(2)}

\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\vu}{\myvec{u}}
\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwh}{\hat{\vw}}
\newcommand{\vx}{\myvec{x}}
\newcommand{\vxh}{\hat{\vx}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
\newcommand{\vy}{\myvec{y}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
\newcommand{\vz}{\myvec{z}}
\newcommand{\vzdiff}{\myvec{z}_{diff}}

\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}


\newcommand{\vxtest}{\myvec{x}_*}
\newcommand{\vytest}{\myvec{y}_*}


\newcommand{\ftrue}{f_{true}}

\newcommand{\myprec}{\mbox{prec}}
\newcommand{\precw}{\lambda_{w}} % precision of weights (alpha)
\newcommand{\precy}{\lambda_{y}} % precision of y (beta)
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}


\newcommand{\htilde}{\tilde{h}}
\newcommand{\vhtilde}{\tilde{\vh}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\pemp}{p_{emp}}
\newcommand{\pstar}{p^*}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\vxtilde}{\tilde{\vx}}
\newcommand{\vytilde}{\tilde{\vy}}
\newcommand{\ztilde}{\tilde{\z}}
\newcommand{\vztilde}{\tilde{\vz}}
\newcommand{\vthetaMAP}{\hat{\vtheta}_{MAP}}
\newcommand{\vthetaS}{\vtheta^{(s)}}
\newcommand{\vthetahat}{\hat{\vtheta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\overline{\theta}}
\newcommand{\vthetabar}{\overline{\vtheta}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\vpibar}{\overline{\vpi}}


\newcommand{\RSS}{\mbox{RSS}}
\newcommand{\mydof}{\mbox{dof}}


\newcommand{\vvec}{\mbox{vec}}
\newcommand{\kron}{\otimes}
\newcommand{\dof}{\mbox{dof}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\energy}{E}
\newcommand{\expectAngle}[1]{\langle #1 \rangle}
\newcommand{\expect}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\expectQ}[2]{\mathbb{E}_{{#2}} \left[ {#1} \right]}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\var}[1]{\mbox{var}\left[{#1}\right]}
\newcommand{\std}[1]{\mbox{std}\left[{#1}\right]}
\newcommand{\varQ}[2]{\mbox{var}_{{#2}}\left[{#1}\right]}
\newcommand{\cov}[1]{\mbox{cov}\left[{#1}\right]}
\newcommand{\median}[1]{\mbox{median}\left[{#1}\right]}

\newcommand{\diag}{\mbox{diag}}
\newcommand{\blkdiag}{\mbox{blkdiag}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}

\newcommand{\size}{\mbox{size}}
\newcommand{\trace}{\mbox{trace}}

\newcommand{\myc}{c}
\newcommand{\myi}{i}
\newcommand{\myj}{j}
\newcommand{\myk}{k}
\newcommand{\myn}{n}
\newcommand{\myq}{q}
\newcommand{\mys}{s}
\newcommand{\myt}{t}


\newcommand{\kernelfn}{\kappa}

\newcommand{\Nsamples}{S}
\newcommand{\Ndata}{N}
\newcommand{\Ndim}{D}
\newcommand{\Nhidden}{H}
\newcommand{\Noutdim}{D_y}
\newcommand{\Nlowdim}{K}
\newcommand{\Nstates}{K}
\newcommand{\Nfolds}{K}
\newcommand{\Npastates}{L}
\newcommand{\Nclasses}{C}
\newcommand{\Nclusters}{K}
\newcommand{\NclustersC}{C}
\newcommand{\Ntime}{T}
\newcommand{\Ntimes}{T}
\newcommand{\Niter}{T}
\newcommand{\Nnodes}{D}

\newcommand{\ki}{i}
\newcommand{\kj}{j}
\newcommand{\kk}{k}
\newcommand{\kC}{C}
\newcommand{\kc}{c}

\newcommand{\supp}{\mbox{supp}}
\newcommand{\query}{\calQ}
\newcommand{\vis}{\calE}
\newcommand{\nuisance}{\calN}
\newcommand{\hid}{\calH}

\newcommand{\advanced}{*}

\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calDx}{{\cal D}_x}
\newcommand{\calE}{{\cal E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calHX}{{\cal H}_X}
\newcommand{\calHy}{{\cal H}_y}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{{\cal NP}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{{\cal L}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{{\cal T}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}

\newcommand{\Lone}{$\ell_1$}
\newcommand{\Ltwo}{$\ell_2$}

\newcommand{\mya}{\mbox{a}}
\newcommand{\myat}{\alpha_{t|t-1}}
\newcommand{\score}{\mbox{score}}
\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\BICcost}{\mbox{BIC-cost}}
\newcommand{\scoreBIC}{\mbox{score-BIC}}
\newcommand{\scoreBICL}{\mbox{score-BIC-L1}}
\newcommand{\scoreL}{\mbox{score-L1}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{do}}
\newcommand{\data}{\calD}
\newcommand{\model}{\calM}
\newcommand{\dataTrain}{\calD_{\mbox{train}}}
\newcommand{\dataTest}{\calD_{\mbox{test}}}
\newcommand{\dataValid}{\calD_{\mbox{valid}}}
\newcommand{\futuredata}{\tilde{\calD}}
\newcommand{\algo}{\calA}
\newcommand{\fitAlgo}{\calF}
\newcommand{\predictAlgo}{\calP}
\newcommand{\err}{\mbox{err}}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\parent}{\mbox{pa}}

\newcommand{\D}{\calD}


\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beaa}{\begin{eqnarray*}}
\newcommand{\eeaa}{\end{eqnarray*}}

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{n}

\newcommand{\vfj}{\vf_j}
\newcommand{\vfk}{\vf_k}

\newcommand{\llbrack}{\left\lbrack}
\newcommand{\rrbrack}{\right\rbrack}
\newcommand{\llbrace}{\left\lbrace}
\newcommand{\rrbrace}{\right\rbrace}
\newcommand{\llpar}{\left(}
\newcommand{\rrpar}{\right)}

\newcommand{\set}[1]{\{#1\}}


==> model.tex <==
\section{The COBRA model}\label{S:model}

\begin{figure*}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/model_schematic_global.png}
  \caption{\textbf{COBRA model schematic}\\
  \textbf{A.} Entire model. The vision module (scene encoder and decoder), transition model, and exploration policy are all trained in a pure exploration phase with no reward. \textbf{B.} Transition model architecture. An action-conditioned slot-wise MLP learns one-step future-prediction. This is trained by applying the scene decoder to $\tilde \vz_{t+1}$, through which gradients from a pixel loss are passed. An auxiliary transition error prediction provides a more direct path to the pixel loss and makes adversarial training with the exploration policy more efficient. \textbf{C.} Adversarial training of transition model and exploration policy through which the behavior of moving objects emerges.
  }
  \label{fig:model_schematic}
  \vspace*{-1em}
\end{figure*}

Our model (Figure~\ref{fig:model_schematic}) consists of four components: The \textbf{vision module}, \textbf{transition model}, and \textbf{exploration policy} are trained during an unsupervised \textit{exploration phase} without rewards, while the \textbf{reward predictor} is trained during a subsequent \textit{task phase} (with reward).

To present the architectures of these components, we must first briefly discuss the environment:
We are interested in environments containing objects that can be manipulated, in which agents can learn purposeful exploration without reward and a diverse distribution of tasks can be defined.
In all of our experiments we use a 2-dimensional virtual ``touch-screen'' environment that contains objects with configurable shape, position, and color.
The agent can move any visible object by clicking on the object and clicking in a direction for the object to move.
Hence the action space is continuous and 4-dimensional, namely a pair of clicks.
If the first click does not land in an object then nothing will move, regardless of the second click.
Despite its apparent simplicity, this environment supports highly diverse tasks that can challenge existing SOTA agents.
See Section \ref{S:env_tasks} for details about our environment and tasks.
We have open-sourced this environment \footnote{Available here: \url{https://github.com/deepmind/spriteworld}}, calling it ``Spriteworld'' \citep{spriteworld}.


\subsection{Unsupervised exploration phase}\label{SS:unsupervised_exploration_phase}

We want our agent to learn how its environment ``works'' in a task-free \textit{exploration phase}, where no extrinsic reward signals are available.
If this is done well, then the knowledge thus gained should be useful and generalizable for subsequent tasks.
Specifically, in the exploration phase COBRA learns representations of objects, dynamics, and its own action space, which it can subsequently use for any task.
For the exploration phase we let COBRA explore our Spriteworld environment in short episodes.
Each episode is initialized with 1-7 objects with randomly sampled shape, position, orientation and color.

\paragraph{Vision Module} We use MONet \citep{burgess2019} to learn a static scene representation.
MONet is an auto-regressive VAE that learns to decompose a scene into entities, such as objects, without supervision.
We can view it as having an encoder $V_{enc}$ and a decoder $V_{dec}$.
The encoder maps an image $\vx$ to a tensor $V_{enc}(\vx) = \vz \in \real^{K \times M}$ representing the full scene.
This representation consists of $K$ entities, each encoded by the mean of MONet's latent distribution of dimension $M$.
We hereafter call each row $k$ of the scene representation $\vz$ a ``slot.''
The decoder maps this tensor $\vz$ to a reconstructed image $V_{dec}(\vz) = \tilde{\vx}$.

Critically, MONet learns to put each object from a scene into a different slot.
Moreover, the MONet architecture ensures that each slot has the same representational semantics, so there is a common learned latent space to which each object is mapped.
Each slot represents meaningful properties of the objects, such as position, angle, color and shape.
See Figure~\ref{fig:supp_disentangling} in Appendix~\ref{S:supp_disentangling} for an example.
MONet can handle scene datasets with a variable number of objects by letting some slots' codes lie in a region of latent space that represents no object.
See Figure \ref{fig:scene_action_transition}-A for scene decomposition results, indicating that MONet successfully learns to accurately represent Spriteworld scenes in terms of objects.

While our Spriteworld environment is visually quite simple, in more complex environments MONet's slots learn to represent other elements of a scene (e.g. backgrounds or walls in 3D scenes) and its latent space can capture more complex visual properties (e.g. surface glossiness).
See \citep{burgess2019} for examples.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.99\linewidth]{figures/scene_action_transition.png}
  \caption{\textbf{Scene decomposition, transition model, and exploration policy results}\\
  \textbf{A.} Vision module (MONet) decomposing Spriteworld scenes into objects (one column per sample scene).
  \textit{(First row)} Data samples.
  \textit{(Second row)} Reconstruction of the full scene.
  \textit{(Other rows)} Individual reconstructions of each slot in the learned scene representation.
  Some slots are decoded as blank images by the decoder.
  \textbf{B.} Rollouts of transition model, treated as an RNN, compared to ground truth on two scenes.
  In each scene, one single item (indicated by dotted circle) is being moved along a line in multiple steps.
  \textbf{C.} Exploration policy.
  \textit{(Left)} Position click component of random samples from the trained exploration policy, which learns to click on (and hence move) objects.
  \textit{(Middle)} Slice through the first two dimensions (position click) of the action sampler's quantile function, showing deformations applied on a grid of first clicks $\in [0, 1]^2$ with randomized second click.
  \textit{(Right)} Slice through second two dimensions (motion click). There is virtually no deformation, indicating the exploration policy learns to sample motions randomly.
  }\label{fig:scene_action_transition}
\end{figure}

\paragraph{Transition model} We introduce a method that maps an action $\va_t$ and a scene representation $\vz_t$ at time step $t$ to a predicted next-step scene representation $\tilde \vz_{t+1}$.
This model applies a shared MLP $T_{net}$ slot-wise to the concatenations $[\vz_t^k; \va_t]$ of each slot $\vz_t^k$ with the action $\va_t$.
This is sufficient to predict $\vz_{t+1}$, because in Spriteworld there are no physical interactions between objects and any action will affect at most one object.
To train this transition model, we cannot easily use a loss in representation space, because the encoding $\vz_{t+1} = V_{enc}(\vx_{t + 1})$ of image $\vx_{t + 1}$ may have a different ordering of its slots than $\vz_t = V_{enc}(\vx_t)$ and solving the resulting matching problem in a general, robust way is non-trivial.
Instead, we circumvent this problem by applying the visual decoder (through which gradients can be passed) to $\tilde \vz_{t+1}$ and using a pixel loss in image space:
\begin{align}
    \tilde \vz_{t+1} = T(\vz_t, \va_t) &= [T_{net}(\vz_t^0, \va_t), ..., T_{net}(\vz_t^K, \va_t)]\nonumber\\
    Loss_{T}(\vz_t, \va_t) &= ||V_{dec}( T(\vz_{t}, \va_t)) - \vx_{t + 1}||^2\nonumber
\end{align}
Additionally, we train an extra network $L_T(\vz, \va)$ to predict the output of the pixel loss, which we use as a measure of curiosity when training the exploration policy, as we found this to work better and be more stable than using the pixel loss directly.
See Appendix~\ref{S:supp_things_tried} for alternative transition models considered, including those that do not use pixel loss.

See Figure \ref{fig:scene_action_transition}-B for examples of transition model rollouts after training in tandem with the exploration policy (covered below).

\paragraph{Exploration Policy} In many environments a uniformly random policy is insufficient to produce action and observation sequences representative of those useful for tasks.
Consequently, in order for a agent to learn through pure exploration a transition model that transfers accurately to a task-driven setting, it should not take uniformly random actions.
In Spriteworld, this manifests itself in the sparseness of the action space.
If an agent were to take uniformly random actions, it would rarely move any object because the agent must click within an object to move it and the objects only take up a small portion of the image ($\approx 1.7 \%$ per object).
This is shown in Figure~\ref{fig:supp_exploration_behaviour} (top) and Appendix~\ref{S:supp_agent_videos}, and our transition model does not get enough examples of objects moving to be trained well in this condition.
Hence we need our agent to learn in the exploration phase a policy that clicks on and moves objects more frequently.

\begin{figure}[t!]
  \centering
  \includegraphics[width=0.55\linewidth]{figures/exploration_before_after_images.png}
  \caption{
  \textbf{Random policy and exploration policy}\\
  Observations and actions taken by an agent during the unsupervised exploratory phase. 
  Actions are shown with small green arrows.
  \textit{(Top)} Random agent, which rarely moves any object, provides a bad source of data for the transition model.
  \textit{(Bottom)} trained exploration policy, which frequently moves objects, provides a good source of data for the transition model.
  }\label{fig:supp_exploration_behaviour}
\end{figure}

Our approach is to train the transition model adversarially with an exploration policy that learns to take actions on which the transition model has a high error.
Such difficult-to-predict actions should be those that move objects (given that others would leave the scene unchanged).
In this way the exploration policy and the transition model learn together in a virtuous cycle.
This approach is a form of curiosity-driven exploration, as previously described in both the psychology \citep{gopnik1999} and the reinforcement learning literature \citep{schmidhuber1990line, schmidhuber1990making, pathak2017curiosity}.
We apply this adversarial training of the transition model and exploration policy in an exploration environment with randomly generated objects (see Appendix~\ref{S:supp_training}).

To put this idea into practice, we must learn a distribution over the 4-dimensional action space from which we can sample.
To do this, we take inspiration from distributional RL \citep{distributional_rl, dabney2017quantile, dabney2018quantile} and learn an approximate quantile function that maps uniform samples $\vu 
\in [0, 1]^4$ to non-uniform samples in our action space $\va \in [0, 1]^4$.
This can be thought of as a perturbation $D$ of each point in $[0, 1]^4$, parameterized by an MLP $D_{net}$.
We train $D_{net}$ to maximize the predicted error $L_T$ of the transition model's prediction of action $\va$, subject to an $L_1$ regularization on the perturbation magnitude. Specifically, given $\vu\in [0, 1]^4$, the exploration policy is trained as:
\begin{align}
    D(\vu, \vz) &= \vu + D_{net}(\vu, \vz) = \va \nonumber\\
    Loss(\vu, \vz) &= |D_{net}(\vu, \vz)| - L_T(\vz, \va)\nonumber
\end{align}
Note that this method does not pressure $D$ to exactly be a quantile function.
Instead it is incentivized to learn a discontinuous approximation of the quantile function.
We tried various approaches to parameterizing $D$ (see Appendix~\ref{S:supp_things_tried}) and found this one to work best.

While the vision module, transition model, and exploration policy can in principle all be trained simultaneously, in practice for the sake of simplicity in this current work we pre-trained the vision module on frames generated by taking random actions in the exploration environment.
We then reloaded this vision module with frozen variables while training the transition model and exploration policy in tandem in the active adversarial exploration phase just described.
See Appendices~\ref{S:supp_model}-\ref{S:supp_training} for architecture and training details.

See Figure \ref{fig:scene_action_transition}-C for examples of samples from the trained exploration policy and a visualization of its deformation.
Images of the exploration policy in action can be seen in Figure~\ref{fig:supp_exploration_behaviour} (bottom), and see Appendix~\ref{S:supp_agent_videos} for videos.


\subsection{Task phase}\label{SS:task_phase}

Once the exploration phase is complete, COBRA enters the \textit{task phase}, in which it is trained to solve several tasks independently.
We freeze the trained vision module, transition model, and exploration policy, training only a separate reward predictor independently for each task.
See Section~\ref{S:env_tasks} for task details.


\paragraph{Reward Predictor}


For each task we train a model-based agent that uses the components learned in the exploration phase and only learns a reward predictor.
The reward predictor is trained from a replay buffer of (\texttt{observation}, \texttt{reward}) pairs, see Algorithm~\ref{alg:agent}.

Our agent acts with a simple 1-step search, sampling a batch of actions from the exploration policy, rolling them out for one step with the transition model, evaluating the predicted states with the reward predictor and selecting the best action (with epsilon-greedy).
This is effectively a myopic 1-step Model Predictive Control (MPC) policy.
It is sufficient to act optimally given the dense rewards in our tasks, but could readily be extended to multi-step MPC, other existing planning algorithms as in \cite{hafner2018learning} or Monte-Carlo Tree Search \citep{alphago}.
Also, see Appendix \ref{S:supp_sparse_rewards} for an extension that works with sparse rewards.


\begin{figure}[t!]
  \centering
  \begin{minipage}{.7\linewidth}
    \begin{algorithm}[H]
    \caption{Task phase agent training}
    \label{alg:agent}
    \begin{algorithmic}
        \REQUIRE Branching factor $B$, Training factor $N$
        \ENSURE Trained reward predictor $R_\theta$
        \STATE $\calR = \varnothing$
        \COMMENT{initialize replay buffer}
        \FOR{$t=1$ {\bfseries to} \texttt{num\_steps}}
        \STATE $\vx_t, r_t = \texttt{environment.obs\_reward()}$
        \STATE $\vz_t = V_{enc}(\vx_t)$
        \COMMENT{scene representation}
        \STATE $\calR \leftarrow \calR \union (\vz_t, r_t)$
        \STATE $\calA = \varnothing$
        \COMMENT{actions and predicted rewards}
        \FOR{$b=1$ {\bfseries to} $B$} 
            \STATE $\vu_b \sim \text{Uniform}([0, 1]^4)$
            \STATE $\va_b = D(\vz_t, \vu_b)$
            \COMMENT{exploration policy action}
            \STATE $\tilde \vz_{t+1} = T(\vz_t, \va_b)$
            \COMMENT{transition model}
            \STATE $\tilde r_b = R_\theta(\tilde \vz_{t+1})$
            \COMMENT{reward predictions}
            \STATE $\calA \leftarrow \calA \union (\va_b, r_b)$
        \ENDFOR
        \STATE $\va = \text{epsilon-greedy}(\max_{\tilde r}(\calA))$
        \COMMENT{best action}
        \STATE $\texttt{environment.step}(\va)$
        \FOR{$i=1$ {\bfseries to} $N$} 
        \STATE $\vz_i, \vr_i \sim \calR$
        \COMMENT{sample minibatch}
        \STATE $\theta \leftarrow \theta - \partial_{\theta} ||R_\theta(\vz_i) - \vr_i||^2$
        \COMMENT{train reward predictor}
        \ENDFOR
        \ENDFOR
    \end{algorithmic}
    \end{algorithm}
  \end{minipage}
\end{figure}
